Multi-armed Bandits with Missing Outcome

While significant progress has been made in designing algorithms that minimize regret in online decision-making, real-world scenarios often introduce additional complexities, perhaps the most challenging of which is missing outcomes. Overlooking this aspect or simply assuming random missingness invariably leads to biased estimates of the rewards and may result in linear regret. Despite the practical relevance of this challenge, no rigorous methodology currently exists for systematically handling missingness, especially when the missingness mechanism is not random. In this paper, we address this gap in the context of multi-armed bandits (MAB) with missing outcomes by analyzing the impact of different missingness mechanisms on achievable regret bounds. We introduce algorithms that account for missingness under both missing at random (MAR) and missing not at random (MNAR) models. Through both analytical and simulation studies, we demonstrate the drastic improvements in decision-making by accounting for missingness in these settings.

==> algorithms/mar_algo1.tex <==
\begin{algorithm}[H]
\caption{MAR Algorithm \( p_{m,a} \)}\label{alg:mar_algorithm2}
\begin{algorithmic}[1]
\State \textbf{Input:} Number of arms $n$, time horizon $T$, $\alpha \geq 1$
\State \textbf{Initialize:} 
\\ Set $\hat{\mu}_{i, a} = 0$ for all arms $a = 1, 2, \dots, n$ and all $i = 1, 2, \dots, K$
\\ Set $n_{i, a} = 0$ for all arms $a$ and all $i \in [K]$ (the number of times arm $a$ is pulled and $M = i$ with the reward observed)
\\ Set $m_{i,a} = 0$ for all arms $a$ and all $i \in [K]$ (the number of times $M = i$ was observed)
\vspace{0.5em}

\For{each arm $a = 1, 2, \dots, n$}
    \For{$T_{1, a}$ rounds}
        \State Pull arm $a$ and observe $m$ and reward $r$
        \State Update $m_{i, a}$ (number of times $M = i$ is observed for arm $a$)
        \If{reward is observed}
            \State Update $n_{a, m}$ and $\hat{\mu}_{a, m}$
        \EndIf
    \EndFor
\EndFor
\vspace{0.5em}

\State $T_1 = \sum\limits_{a} T_{1, a}$
\State $T_2 = T - T_1$

\vspace{0.5em}
\For{each round $t = 1, 2, \dots, T_2$}
    \For{each arm $a = 1, 2, \dots, n$}
        \State Estimate \( p_{m,a} = \frac{m_{i,a}}{T_a} \) for each $i \in [K]$
        \vspace{0.5em}
        \State Compute $\hat{\mu}_{a} = \sum\limits_{i \in [K]} p_{m,a} \hat{\mu}_{i, a}$
        \State Compute $\text{UCB}_a(t) = \hat{\mu}_a + \sqrt{\frac{\alpha \log t}{2}} \sum\limits_{i \in [K]} p_{m,a} \sqrt{\frac{1}{n_{i,a}}}$
    \EndFor
    \State Select arm $a_t = \arg \max_a \text{UCB}_a(t)$
    \State Pull arm $a_t$ and observe $m$ and reward $r_t$
    \State Update $m_{i,a_t}$ (number of times $M = i$ is observed for arm $a_t$)
    \If{reward is observed}
        \State Update $n_{a_t, m}$ and $\hat{\mu}_{a_t, m}$
    \EndIf
\EndFor

\end{algorithmic}
\end{algorithm}


==> proofs/db.tex <==
\begin{proof}
First assume that the missingness probabilities are consistently estimated.
That is, \( \hat{\gamma}_{m, a} \) are consistent estimators for \(\gamma_{m,a}\). 
We have \( \forall \epsilon \):
\[
\lim\limits_{T \rightarrow \infty} \mathbb{P}(|\hat{\gamma}_{m, a} - \gamma_{m, a}| \geq \epsilon) = 0
\]

We have with probability \( 1 - \mathbb{P}(|\hat{\gamma}_{m, a} - \gamma_{m, a}| \geq \epsilon)\) that:
\[
|\hat{\gamma}_{m, a} - \gamma_{m, a}| \leq \epsilon
\]
so
\begin{align*} 
    |\frac{1}{\hat{\gamma}_{m, a}} - \frac{1}{\gamma_{m, a}}| \leq \frac{\epsilon}{\gamma_{m, a} \hat{\gamma}_{m, a}} 
    \leq \frac{\epsilon}{\gamma_{m, a} (\gamma_{m, a} - \epsilon)}
\end{align*}

Now we have:
\begin{equation}
    \label{eq:db_1}
    \hat{\mu}_a = \sum\limits_{t = 1}^T\big[
        \sum_{m\in\mathcal{M}}\frac{\mathbbm{1}\{M_t=m\}}{\hat{\gamma}_{m,a}}\big(
        Y^o_t\mathbbm{1}\{\oo_t=1\}-(\mathbbm{1}\{\oo_t=1\}-\hat{\gamma}_{m,a})\hat{\mu}_{m, a} = O(\epsilon)
    \big]
\end{equation}


Now if \( T_{m, o} \) be the number of times \(M = m \) and reward observed and \( T_{m, o'}\) be the number of times \(M = m \) observed and reward missed then: 
\begin{align*}
    \hat{\mu}_a 
    &= \sum\limits_{m \in \mathbb{M}} \big[
    T_{m, o'} \hat{\mu}_{m, a} 
    -\frac{1 - \hat{\gamma}_{m, a}}{\hat{\gamma}_{m, a}} T_{m, o} \hat{\mu}_{m, a}
    + \frac{1}{\hat{\gamma}_{m, a}} \sum\limits_{t_1 = 1}^{T_{m, o}} Y^o_t
    \big] \\
    &= \sum\limits_{m \in \mathbb{M}} \big[
    \hat{\mu}_{m, a} (T_m - \frac{1}{\hat{\gamma}_{m, a}}T_{m, o})
    + \frac{1}{\hat{\gamma}_{m, a}} \sum\limits_{t_1 = 1}^{T_{m, o}} Y^o_t
    \big] 
 \end{align*}

Now using \ref{eq:db_1} with probability \( 1 - \sum\limits_{m \in \mathbb{M}} \mathbb{P}(|\hat{\gamma}_{m, a} - \gamma_{m, a}| \geq \epsilon)\) we will have:
\[
\hat{\mu}_a = \sum\limits_{m \in \mathbb{M}} \big[
    \hat{\mu}_{m, a} (T_m - \frac{1}{\gamma_{m, a}}T_{m, o})
    + \frac{1}{\gamma_{m, a}} \sum\limits_{t_1 = 1}^{T_{m, o}} Y^o_t
    \big] + O(\epsilon)
\]

Now using Chebyshev's inequality we have:
\[
\mathbb{P}(|\frac{T_{m, o}}{T_m} - \gamma_{m, a}| \geq \frac{\epsilon \gamma_{m, a}}{T_m}) \leq \frac{\gamma_{m, a} (1 - \gamma_{m, a})}{T_m \epsilon \gamma_{m, a}}
\]
which yields:
\[
\mathbb{P}(|\frac{T_{m, o}}{\gamma_{m, a}} - {T_m}| \geq \epsilon) \leq \frac{(1 - \gamma_{m, a})}{T_m \epsilon}
\]

\end{proof}
